Hierarchical Nearest Neighbor Graph Embedding for Efficient Dimensionality Reduction

Dimensionality reduction is crucial both for visualization and preprocessing high dimensional data for machine learning. We introduce a novel method based on a hierarchy built on 1-nearest neighbor graphs in the original space which is used to preserve the grouping properties of the data distribution on multiple levels. The core of the proposal is an optimization-free projection that is competitive with the latest versions of t-SNE and UMAP in performance and visualization quality while being an order of magnitude faster in run-time. Furthermore, its interpretable mechanics, the ability to project new data, and the natural separation of data clusters in visualizations make it a general purpose unsupervised dimension reduction technique. In the paper, we argue about the soundness of the proposed method and evaluate it on a diverse collection of datasets with sizes varying from 1K to 11M samples and dimensions from 28 to 16K. We perform comparisons with other state-of-the-art methods on multiple metrics and target dimensions highlighting its efficiency and performance. Code is available at https://github.com/koulakis/h-nne

==> tab/algorithm_projection.tex <==
\begin{algorithm}
\caption{Hierarchical point translation}\label{alg:projection}
\begin{algorithmic}
% \Input {A list of sets of anchors $A$ for each level of the hierarchy, starting from the top level and ending with the actual datapoints}
\State $anc \gets anchors[1]$\;

\For{$lowanc$\ in\ anchors[1:], mapping in levels}
\State $anc \gets move(lowanc, anc, mapping)$
\EndFor
\State $points \gets anc$
\end{algorithmic}
\end{algorithm}
%     curr_anchors = projected_anchors[-1]
%     for i in reversed_partition_range:
%         if i == 0:
%             partition_mapping = partitions[:, 0]
%         else:
%             partition_mapping = partition_labels[i - 1]
        
        
%         current_points = projected_anchors[i]
        
%         curr_anchors, radii = move_projected_points_to_anchors(
%             current_points,
%             curr_anchors, 
%             partition_mapping, 
%             first_neighbors_list[i],
%             radius_shrinking=curr_radius_shrinking,
%             real_nn_threshold=real_nn_threshold,
%         )
        
        
        
% if anchors.shape[0] <= real_nn_threshold:
%         distance_matrix = pairwise.pairwise_distances(anchors, anchors, metric='euclidean')
%         np.fill_diagonal(distance_matrix, 1e12)
%         nearest_neighbor_idx = np.argmin(distance_matrix, axis=1).flatten()
%     else:
%         print('Using ann to approximate 1-nns...')
%         knn_index = NNDescent(
%             anchors, 
%             n_neighbors=2, 
%             metric='euclidean', 
%             verbose=True, 
%             low_memory=True)
%         nns, _ = knn_index.neighbor_graph
%         nearest_neighbor_idx = nns[:, 1]
        
%     anchor_radii = np.linalg.norm(anchors - anchors[nearest_neighbor_idx], axis=1, keepdims=True)
%     anchor_radii = anchor_radii / 2 * radius_shrinking
    
%     anchors_per_point = anchors[partition]
%     anchor_radii_per_point = anchor_radii[partition]
    
%     points_mean = cool_mean(points, partition)[partition]
%     points_centered = points - points_mean

%     points_max_radius = np.expand_dims(cool_max_radius(points_centered, partition), axis=1)
%     points_max_radius = np.where(points_max_radius == 0, 1., points_max_radius)
    
%     return anchors_per_point + anchor_radii_per_point * points_centered / points_max_radius, anchor_radii[:, 0].tolist()
